Joint Debiased Representation and Image Clustering Learning with Self-Supervision

Contrastive learning is among the most successful methods for visual representation learning, and its performance can be further improved by jointly performing clustering on the learned representations. However, existing methods for joint clustering and contrastive learning do not perform well on long-tailed data distributions, as majority classes overwhelm and distort the loss of minority classes, thus preventing meaningful representations to be learned. Motivated by this, we develop a novel joint clustering and contrastive learning framework by adapting the debiased contrastive loss to avoid under-clustering minority classes of imbalanced datasets. We show that our proposed modified debiased contrastive loss and divergence clustering loss improves the performance across multiple datasets and learning tasks. The source code is available at https://anonymous.4open.science/r/SSL-debiased-clustering

==> chapters/justification.tex <==



\subsection{Justification of Over-Clustering}
Let $\tilde{\mathcal{L}}_{deb}^{mod}$ denote the loss of the image $x_i$ to a positive sample $x^+$:

\begin{align}
\tilde{\mathcal{L}}_{deb}^{mod} = log \frac{exp(sim(\Tilde{z}_i, \Tilde{z}^+)/\tau)}{exp(sim(\Tilde{z}_i, \Tilde{z}^+)/\tau) + Neg^{\lambda_{mod}}_i} \\
\end{align}

\begin{align*}
    \frac{\partial \tilde{\mathcal{L}}_{deb}^{mod}}{\partial \lambda_{mod}} =& \frac{\partial}{\partial \lambda_{mod}} log\big[exp(sim(\Tilde{z}_i, \Tilde{z}^+)/\tau) \\
    &+ (1 + \sum_{j=1}^{2N-2} exp(sim(\Tilde{z}_i, z^{Neg}_j)/\tau))^{\lambda_{mod}}\big] \\
    &- log\big[exp(sim(\Tilde{z}_i, \Tilde{z}^+)/\tau)\big] \\
    =& \big(exp(sim(\Tilde{z}_i, \Tilde{z}^+)/\tau) \\
    &+ (1 + \sum_{j=1}^{2N-2} exp(sim(\Tilde{z}_i, z^{Neg}_j)/\tau))^{\lambda_{mod}}\big)^{-1} \\
    &* (1 + \sum_{j=1}^{2N-2} exp(sim(\Tilde{z}_i, z^{Neg}_j)/\tau))^{\lambda_{mod}}) \\
    &* log\big[1 + \sum_{j=1}^{2N-2} exp(sim(\Tilde{z}_i, z^{Neg}_j)/\tau))^{\lambda_{mod}} \big]
\end{align*}
\begin{align*}
    \frac{\partial^2 \tilde{\mathcal{L}}_{deb}^{mod}}{\partial^2 \lambda_{mod}}=& exp(sim(\Tilde{z}_i, \Tilde{z}^+)/\tau) \\
    &* (1 + \sum_{j=1}^{2N-2} exp(sim(\Tilde{z}_i, z^{Neg}_j)/\tau))^{\lambda_{mod}}\\
    &*log\big[ 1 + \sum_{j=1}^{2N-2} exp(sim(\Tilde{z}_i, z^{Neg}_j)/\tau)) \big]^2\\
    &* \Big[exp(sim(\Tilde{z}_i, \Tilde{z}^+)/\tau) \\
    &+ (1 + \sum_{j=1}^{2N-2} exp(sim(\Tilde{z}_i, z^{Neg}_j)/\tau))^{\lambda_{mod}}\Big]^{-2}
\end{align*}
\begin{align*}
    lim_{sim(\Tilde{z}_i, z^{Neg}_j) \to 0, \forall j \in (2N-2)}& \frac{\partial^2 \tilde{\mathcal{L}}_{deb}^{mod}}{\partial^2 \lambda_{mod}} = \\
    exp(sim(\Tilde{z}_i, \Tilde{z}^+)/\tau) \\
    &* (2N-1)^{\lambda_{mod}}\\
    &*log\big[ 2N - 1) \big]^2\\
    &* \Big[exp(sim(\Tilde{z}_i, \Tilde{z}^+)/\tau) \\
    &+ (2N- 1))^{\lambda_{mod}}\Big]^{-2}
\end{align*}

\begin{align*}
    lim_{sim(\Tilde{z}_i, \Tilde{z}^+) \to 1}& \frac{\partial^2 \tilde{\mathcal{L}}_{deb}^{mod}}{\partial^2 \lambda_{mod}} = exp(1)/\tau) * (\eta)^{\lambda_{mod}}\\
    &*log\big[ \eta \big]^2 * \Big[exp(1/\tau) + \eta)^{\lambda_{mod}}\Big]^{-2}
\end{align*}

Assuming that the negative samples for the image $x_i$ are not completely unsimilar, that is the case if the representation generated by $h_{\Tilde{\theta}}$ are orthogonal to each other, it follows $\eta >> (2N -1)$


==> tables/analyis_K.tex <==
%---------------------------------------------------
%     Impact of K
%---------------------------------------------------
\begin{table*} [!t]
%\vspace{-3pt}
\centering
\caption{Top-1 accuracy (in \%) under linear evaluation when our method is trained on top of different numbers of subnetworks and using CIFAR-10 ($\kappa$) data. The performance of the divergence learning framework depends on the representation feature space, while our method significantly outperforms deep divergence.}
%\vspace{-2pt}
%\small
\label{table:lineareval:k}
\begin{tabular}{l l l l l l l l }
\toprule
Number of subnetworks $\bm k$ & 5 & 20 & 50 & 100 & 200 & 500 & 1000 \\
\midrule
Deep Divergence~\cite{cilingir2020deep} & 71.9 & 77.8 & 79.4 & 80.0 & 77.4 & 74.1 & 70.8 \\
Our Method                              & 85.2 & 88.9 & 91.0 & 92.6 & 92.8 & 89.2 & 85.5 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/clustering_evaluation.tex <==
%---------------------------------------------------
%     Table Unsupervised Clustering Evaluation Dataset
%---------------------------------------------------
\begin{table*} 
\centering
\small
\caption{Comparison of the proposed method with the baseline on image clustering measured by top-1 accuracy (\%) and F1-score.} 
\label{table:clusteringeval}
\begin{tabular}{l| c c c c c c c}
\toprule
Method  & ISIC & Glaucoma-1 & Glaucoma-2 & CIFAR-10 & Imb-CIFAR-10 & CIFAR-100 & Imb-CIFAR-100 \\
\midrule
SimCLR~\cite{chen_simple_2020}      & 47.01 $\pm$ 1.12 & 82.92 $\pm$ 0.20 & 90.00 $\pm$ 0.00  & 78.41 $\pm$ 0.42 & 79.00 $\pm$ 0.26 & 47.75 $\pm$ 0.13 & 45.29 $\pm$ 0.13 \\
(F-1 Score) & (14.71 $\pm$ 0.26) & (78.83 $\pm$ 0.08) & (40.00 $\pm$ 0.00) & (78.26 $\pm$ 0.41) & (51.02 $\pm$ 1.96) & (48.94 $\pm$ 0.10) & (26.09 $\pm$ 0.48) \\
SimSiam~\cite{chen2021exploring}     & 48.01 $\pm$ 1.55 & 79.31 $\pm$ 1.77 & 86.67 $\pm$ 0.00 & 74.96 $\pm$ 0.36 & 74.94 $\pm$ 0.17 & 42.62 $\pm$ 0.55 & 40.53 $\pm$ 0.10 \\
(F-1 Score) & (13.59 $\pm$ 0.33) & (82.78 $\pm$ 0.40) & (38.1 $\pm$ 6.74) & (74.90 $\pm$ 0.39) & (45.89 $\pm$ 1.15) & (47.70 $\pm$ 0.12) & 22.47 $\pm$ 1.08 \\
Debiased~\cite{chuang_debiased_2020}    & 47.34 $\pm$ 0.23 & 84.31 $\pm$ 1.38 & (89.17 $\pm$ 1.18) & 80.13 $\pm$ 0.17 & 80.07 $\pm$ 0.35 & 49.03 $\pm$ 0.07 & 45.80 $\pm$ 0.33 \\ 
(F-1 Score) & (13.91 $\pm$ 0.54) & (80.56 $\pm$ 1.56) & (38.18 $\pm$ 2.57) & (80.00 $\pm$ 0.17) & (50.51 $\pm$ 0.20) & (48.94 $\pm$ 0.10) & (26.09 $\pm$ 0.48) \\\hline
Our method  & \textbf{49.10 $\pm$ 0.23} & \textbf{82.78 $\pm$ 0.40} & \textbf{88.33 $\pm$ 0.00} & \textbf{81.17 $\pm$ 0.34} & \textbf{79.83 $\pm$ 0.97} & \textbf{49.82 $\pm$ 0.11} & \textbf{47.72 $\pm$ 0.00} \\
(F-1 Score) & (15.26 $\pm$ 0.05) & (78.76 $\pm$ 1.00) & (36.36 $\pm$ 0.00) & (81.09 $\pm$ 0.33) & (51.84 $\pm$ 2.26) & (49.82 $\pm$ 0.11) & 27.15 $\pm$ 0.27 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/transfer_learning.tex <==
%---------------------------------------------------
%     Table Transfer Learning Evaluation Dataset
%---------------------------------------------------
\begin{table*} 
\small
\centering
\caption{Comparison of the proposed method with the baseline on transfer learning measured by top-1 accuracy (\%) and F1-score.} 
\label{table:transferlearning}
\begin{tabular}{l| c c}
\toprule
Method   & Glaucoma-1 to Glaucoma-2 & Glaucoma-2 to Glaucoma-1  \\
\midrule
SimCLR      & 88.33 & 75.28 \\
SimSiam     & 88.33 & 71.94 \\
Debiased    & 88.33 & 77.22 \\ \hline
Our method  & 88.33 & 73.89 \\ 
\bottomrule
\end{tabular}
\end{table*}
